Measuring Compliance of Consent Revocation on the Web

The GDPR requires websites to facilitate the right to revoke consent from Web users. While numerous studies measured compliance of consent with the various consent requirements, no prior work has studied consent revocation on the Web. Therefore, it remains unclear how difficult it is to revoke consent on the websites' interfaces, nor whether revoked consent is properly stored and communicated behind the user interface. Our work aims to fill this gap by measuring compliance of consent revocation on the Web on the top-200 websites. We found that 19.87% of websites make it difficult for users to revoke consent throughout different interfaces, 20.5% of websites require more effort than acceptance, and 2.48% do not provide consent revocation at all, thus violating legal requirements for valid consent. 57.5% websites do not delete the cookies after consent revocation enabling continuous illegal processing of users' data. Moreover, we analyzed 281 websites implementing the IAB Europe TCF, and found 22 websites that store a positive consent despite user's revocation. Surprisingly, we found that on 101 websites, third parties that have received consent upon user's acceptance, are not informed of user's revocation, leading to the illegal processing of users' data by such third parties. Our findings emphasise the need for improved legal compliance of consent revocation, and proper, consistent, and uniform implementation of revocation communication and data deletion practices.

==> possible_violations.tex <==
\section{Possible violations}

As discussed in the section \ref{sec:legal_bg}, there are different requirements that the data controllers, websites and third-party vendors have to provide for a data subject to be able to withdraw their initially given consent. 

\GKcom{To do for gayatri}

\subsubsection{Websites must provide information about how consent can
be withdrawn.} 

The websites are required to give the data subject information about how to withdraw before they even give consent. 
We observe that \_\_ consent banners,on the initial landing, indicate where the user can find the option to withdraw or modify after they give the consent. Some websites \_\_ provided this information on the privacy and cookie policy pages. 

Additonally, once the consent is given, we observed that some websites have a alert or popup indicating the directions to modify the consent. While this might be very informative, we observed that a very less no.of websites \_\_ had this functionality. 

\todo{\subsubsection{Withdrawal should be facilitated at all times.} Location? We don't check this right now}

\noindent \textbf{Consent withdrawal must be easy} The legal requirement is that withdrawal should be as easy as giving consent. However as observed in section \ref{sec:results2}, the table is indicative of the inconsistencies in the ease of giving consent as well as withdrawal. 

\noindent \textbf{Consent withdrawal should be non-detrimental} If the data subject rejects or revokes their consent, the functionality and quality of service from the website should not be affected. \textcolor{red}{We can maybe compare the no.of functionality related cookies being decreased}

\noindent \textbf{Data processed before withdrawal is not affected however, Withdrawal means stopping data processing, and consent-
based data must be deleted.} 

The results in section \ref{sec:results4} indicate that majority of the websites have an increase in the number of cookies after revoking their consent. We categorise the cookie into functional, advertising and marketing cookies in order to determine the purpose for them to be either added or left even after the consent is being withdrawn. 

\textcolor{red}{ Cookie categorization table}

\noindent \textbf{Communication of withdrawal to third parties}

\textcolor{red}{See the requests with cookies either regex consent,privacy,grdp etc.}

\noindent \textbf{Design of withdrawal}

\textbf{\textit{Element of withdrawal:}} As discussed in section \ref{sec:results1}, there are different explicit ways to provide a withdrawal option. Privacy pages have toggle switches, buttons, checkboxes or could just open a privacy banner. We observed that \_\_ only have icons opening the privacy management centre. 

\textbf{\textit{Location of withdrawal:}} Similarly, the methods discussed also varied on where these options are placed. In section \ref{sec:results1}, we discussed that there could be a direct option on the footer, or in the privacy page. However, when on the privacy page, the links to popups,toggle switches, buttons, checkboxes can be between texts as well. 
This again indicates the inconsistencies in the way withdrawal options can be found by the data subject on the privacy/cookie policy pages. 

\textbf{\textit{Path to withdrawal:}} Again, the methods in \ref{sec:results1} are indicative of the fact that the option of withdrawal can be present anywhere on the privacy and cookie policy pages. There are \_\_ websites where it might take multiple steps to reach the option to opt-out. 

\textcolor{red}{Add a graph/table indicating the no.of steps taken to reach the withdrawal option.} 

\textbf{\textit{Text of withdrawal:}} We observed different keywords being used, in all the methods mentioned in section \ref{sec:results1}. While they are still indicative of the purpose of withdrawal, some the texts and links leading to withdrawal options were found to be very lucrative and difficult to find for a data subject. 

\textcolor{red}{give examples in every case}

==> tables/data_analysis2.tex <==
\begin{table*}[b]
  \centering
  \includegraphics[width=\linewidth]{plots/225.pdf}
  \caption{Prevalence and type of consent revocation options on 200 to 5000 ranked websites \emph{with} detected CMPs}
  \label{tab:data_analysis3}  
\end{table*}

% \begin{table*}[]
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{|lrrrrrlrrrrrr|}
% \hline
% \multicolumn{13}{|c|}{\textbf{With Detected CMP (1000 from Top 200-5000)}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   \\ \hline
% \multicolumn{1}{|c|}{}                                  & \multicolumn{1}{c|}{}                                           & \multicolumn{5}{c|}{\textbf{Within the Same Interface}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          & \multicolumn{4}{c|}{\textbf{Via Different Interfaces}}                                                                                                                                                                                                                                                                                    & \multicolumn{2}{c|}{\textbf{No Revocation}}                                                                                                                                                              \\ \cline{3-13} 
% \multicolumn{1}{|c|}{\multirow{-2}{*}{\textbf{Banner}}} & \multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{No. of Websites}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9EAD3}\textbf{\begin{tabular}[c]{@{}c@{}}Persistent Icon \\ or Button\\  (0 Steps)\end{tabular}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9EAD3}\textbf{\begin{tabular}[c]{@{}c@{}}Footer Options\\ \\ (1 Step)\end{tabular}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9EAD3}\textbf{\begin{tabular}[c]{@{}c@{}}Banner on Policy\\ \\ (1 step)\end{tabular}}} & \multicolumn{2}{c|}{\cellcolor[HTML]{FFF2CC}\textbf{\begin{tabular}[c]{@{}c@{}}Options through\\  Policy Page\\ (≥ 2 steps)\end{tabular}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EA9999}\textbf{\begin{tabular}[c]{@{}c@{}}Browser set., \\ 3rd-party links\end{tabular}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EA9999}\textbf{After Login}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EA9999}\textbf{Contact/Email}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EA9999}\textbf{Paywalls}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EA9999}\textbf{\begin{tabular}[c]{@{}c@{}}Option mentioned\\  but doesn't work\end{tabular}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{EA9999}\textbf{No revocation}} \\ \hline
% \multicolumn{1}{|l|}{Consent Banner}                    & \multicolumn{1}{r|}{214}                                        & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}33}                                                                                         & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}125}                                                                           & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}0}                                                                               & \multicolumn{2}{r|}{\cellcolor[HTML]{FFF2CC}26}                                                                                            & \multicolumn{1}{r|}{\cellcolor[HTML]{EA9999}9}                                                                                 & \multicolumn{1}{r|}{\cellcolor[HTML]{EA9999}0}                    & \multicolumn{1}{r|}{\cellcolor[HTML]{EA9999}3}                      & \multicolumn{1}{r|}{\cellcolor[HTML]{EA9999}11}                & \multicolumn{1}{r|}{\cellcolor[HTML]{EA9999}3}                                                                                     & \cellcolor[HTML]{EA9999}7                                           \\ \hline
% \multicolumn{1}{|l|}{No Option Banner}                  & \multicolumn{1}{r|}{0}                                          & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}0}                                                                                          & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}0}                                                                             & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}0}                                                                               & \multicolumn{2}{r|}{\cellcolor[HTML]{FFF2CC}0}                                                                                             & \multicolumn{1}{r|}{\cellcolor[HTML]{EA9999}0}                                                                                 & \multicolumn{1}{r|}{\cellcolor[HTML]{EA9999}0}                    & \multicolumn{1}{r|}{\cellcolor[HTML]{EA9999}0}                      & \multicolumn{1}{r|}{\cellcolor[HTML]{EA9999}0}                 & \multicolumn{1}{r|}{\cellcolor[HTML]{EA9999}0}                                                                                     & \cellcolor[HTML]{EA9999}0                                           \\ \hline
% \multicolumn{1}{|l|}{No Banner}                         & \multicolumn{1}{r|}{11}                                         & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}0}                                                                                          & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}8}                                                                             & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}0}                                                                               & \multicolumn{2}{r|}{\cellcolor[HTML]{FFF2CC}0}                                                                                             & \multicolumn{1}{r|}{\cellcolor[HTML]{EA9999}1}                                                                                 & \multicolumn{1}{r|}{\cellcolor[HTML]{EA9999}0}                    & \multicolumn{1}{r|}{\cellcolor[HTML]{EA9999}0}                      & \multicolumn{1}{r|}{\cellcolor[HTML]{EA9999}0}                 & \multicolumn{1}{r|}{\cellcolor[HTML]{EA9999}0}                                                                                     & \cellcolor[HTML]{EA9999}2                                           \\ \hline
% \multicolumn{1}{|l|}{\textbf{Total}}                    & \multicolumn{1}{r|}{225}                                        & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}33}                                                                                         & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}133}                                                                           & \multicolumn{1}{r|}{\cellcolor[HTML]{D9EAD3}0}                                                                               & \multicolumn{2}{r|}{\cellcolor[HTML]{FFF2CC}26}                                                                                            & \multicolumn{1}{r|}{\cellcolor[HTML]{EA9999}10}                                                                                & \multicolumn{1}{r|}{\cellcolor[HTML]{EA9999}0}                    & \multicolumn{1}{r|}{\cellcolor[HTML]{EA9999}3}                      & \multicolumn{1}{r|}{\cellcolor[HTML]{EA9999}11}                & \multicolumn{1}{r|}{\cellcolor[HTML]{EA9999}3}                                                                                     & \cellcolor[HTML]{EA9999}9                                           \\ \hline
% \end{tabular}
% }
% \caption{Prevalence of Consent Banners on Websites with Detected CMP (200 to 5000 rank)}

% \end{table*}

==> tables/purposes.tex <==
% \begin{table*}
{\scriptsize
\onecolumn
% \begin{adjustbox}{width=\linewidth}
\begin{longtable}{|p{2cm}|p{2cm}|p{6cm}|p{1cm}|p{4cm}|}
\hline
\textbf{Purpose}                                    & \textbf{Name}                                                                          & \textbf{Description of the purpose}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      & \textbf{Repeated from v2.0}                                                                                  & \textbf{Requires Consent}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             \\ \hline
1                                                   & Store and/or access information on a device                                            & Cookies, device or similar online identifiers (e.g. login-based identifiers, randomly assigned identifiers, network based identifiers) together with other information (e.g. browser type and information, language, screen size, supported technologies etc.) can be stored or read on your device to recognise it each time it connects to an app or to a website, for one or several of the purposes presented here.                                                                                                                                                                                                                                                                  & \begin{tabular}[c]{@{}l@{}}=\\ 1\end{tabular}                                                                   & \cmark                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      \\ \hline
2                                                   & Use limited data to select advertising                                                 & Advertising presented to you on this service can be based on limited data, such as the website or app you are using, your non-precise location, your device type or which content you are (or have been) interacting with (for example, to limit the number of times an ad is presented to you)                                                                                                                                                                                                                                                                                                                                                                                          & New Looks new language but related to no.2 = “Select basic ads”       & \cmark                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      \\ \hline
3                                                   & Create profiles for personalised advertising                                           & Information about your activity on this service (such as forms you submit, content you look at) can be stored and combined with other information about you (for example, information from your previous activity on this service and other websites or apps) or similar users. This is then used to build or improve a profile about you (that might include possible interests and personal aspects). Your profile can be used (also later) to present advertising that appears more relevant based on your possible interests by this and other entities.                                                                                                                             & \begin{tabular}[c]{@{}l@{}}=\\ 3\end{tabular}                                                                   & \cmark                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      \\ \hline
4                                                   & Use profiles to select personalised advertising                                        & Advertising presented to you on this service can be based on your advertising profiles, which can reflect your activity on this service or other websites or apps (like the forms you submit, content you look at), possible interests and personal aspects.                                                                                                                                                                                                                                                                                                                                                                                                                             & \begin{tabular}[c]{@{}l@{}}=\\ 4\end{tabular}                                                                   & \cmark                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     \\ \hline
\begin{tabular}[c]{@{}l@{}}5\\ \end{tabular} & Create profiles to personalise content                                                 & Information about your activity on this service (for instance, forms you submit, non-advertising content you look at) can be stored and combined with other information about you (such as your previous activity on this service or other websites or apps) or similar users. This is then used to build or improve a profile about you (which might for example include possible interests and personal aspects). Your profile can be used (also later) to present content that appears more relevant based on your possible interests, such as by adapting the order in which content is shown to you, so that it is even easier for you to find content that matches your interests. & \begin{tabular}[c]{@{}l@{}}=\\ 5\end{tabular}                                                                   & (\cmark) Not clear: in principle, this purpose can be legitimized under a legitimate interest, but it would fail the this test.  %. However, according to Recital 47 of the GPDR, when using legitimate interest as a legal basis for processing, the controller (in the balance test) has to consider the reasonable expectations of data subjects based on their relationship with the controller. This expectation must exist at the time and in the context of the collection of her personal data. Meanwhile, the collection of data from unknown sources, by third-parties that users have never heard of and do not have a direct relationship with – to profile them and share these “insights” with other advertisers – is not plausibly within the individuals’ reasonable expectations. Hence, we suppose that processing personal data of users that have no relationship with third-party advertisers, which is the case in the TCF, will, in practice, make that balance weight towards the interest and rights of users. As posited by the Norwegian Consumer Council , “although consumers may know that many “free” digital services are funded by advertising, this does not mean that most people will have a “reasonable expectation” of the amount of sharing and processing going on behind the scenes (...) Companies are virtually unknown to most consumers, so one can hardly consider this a relationship at all.” Thus, the potentially unique purpose (from the specification of the TCF) that would rely on legitimate interest could, in practice, fail the requirements of such a legal basis. 
\\ \hline
6                                                   & Use profiles to select personalised content                                            & Content presented to you on this service can be based on your content personalisation profiles, which can reflect your activity on this or other services (for instance, the forms you submit, content you look at), possible interests and personal aspects. This can for example be used to adapt the order in which content is shown to you, so that it is even easier for you to find (non-advertising) content that matches your interests.                                                                                                                                                                                                                                         & \begin{tabular}[c]{@{}l@{}}=\\ 6\end{tabular}                                                                   & (\cmark) Not clear: in principle, this purpose can be legitimized under a legitimate interest, but it would fail the legitimate interest test.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   \\ \hline
7                                                   & Measure advertising performance                                                        & Information regarding which advertising is presented to you and how you interact with it can be used to determine how well an advert has worked for you or other users and whether the goals of the advertising were reached. For instance, whether you saw an ad, whether you clicked on it, whether it led you to buy a product or visit a website, etc. This is very helpful to understand the relevance of advertising campaigns.                                                                                                                                                                                                                                                    & \begin{tabular}[c]{@{}l@{}}=\\ 7\end{tabular}                                                                   & \cmark                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      \\ \hline
8                                                   & Measure content performance                                                            & Information regarding which content is presented to you and how you interact with it can be used to determine whether the (non-advertising) content e.g. reached its intended audience and matched your interests. For instance, whether you read an article, watch a video, listen to a podcast or look at a product description, how long you spent on this service and the web pages you visit etc. This is very helpful to understand the relevance of (non-advertising) content that is shown to you.                                                                                                                                                                               & \begin{tabular}[c]{@{}l@{}}=\\ 8\end{tabular}                                                                   & \cmark                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      \\ \hline
9                                                   & Understand audiences through statistics or combinations of data from different sources & Reports can be generated based on the combination of data sets (like user profiles, statistics, market research, analytics data) regarding your interactions and those of other users with advertising or (non-advertising) content to identify common characteristics (for instance, to determine which target audiences are more receptive to an ad campaign or to certain contents).                                                                                                                                                                                                                                                                                                  & New language but Looks like the former purpose no. 9 ‘’Apply market research to generate audience insights’’ & \cmark                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      \\ \hline
10                                                  & Develop and improve services                                                           & Information about your activity on this service, such as your interaction with ads or content, can be very helpful to improve products and services and to build new products and services based on user interactions, the type of audience, etc. This specific purpose does not include the development or improvement of user profiles and identifiers.                                                                                                                                                                                                                                                                                                                                & \begin{tabular}[c]{@{}l@{}}= \\ 10\end{tabular}                                                                 & It is not specific, and so we cannot derive its legal basis. \newline \newline X but in principle it could rely on LI though it could fail the LI test                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     \\ \hline
11                                                  & Use limited data to select content                                                     & Content presented to you on this service can be based on limited data, such as the website or app you are using, your non-precise location, your device type, or which content you are (or have been) interacting with (for example, to limit the number of times a video or an article is presented to you).                                                                                                                                                                                                                                                                                                                                                                            & New                                                                                                             & X                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      \\ \hline
% \end{tabular}
    
% \end{adjustbox}
\caption{IAB TCF purposes in v2.2 in the \tcs and the applicable legal basis. The ``Requires Consent'' column sums up our analysis. The ``Repeated from v2.0.'' column compares the purposes of versions v2.0 and v2.2. We add parentheses if exceptions occur.
You can find the descriptions of all the purposes in the Supplemental Material~\cite{INSERT}. \NBtext{move this to supplemental and remove the purpose description}
}
\label{tab:purposes}
\end{longtable}
}

==> tables/purposes2.tex <==
\begin{table*}[h]
\footnotesize
% \onecolumn
\begin{tabular}{|l|p{3cm}|p{4cm}|p{7cm}|}
% \begin{tabular}
\hline
\textbf{Purpose}                                    & \textbf{Name}                                                                          & \textbf{Repeated P from v 2.0}                                                                                  & \textbf{Requires Consent?}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             \\ \hline
1                                                   & Store and/or access information on a device                                            & \begin{tabular}[c]{@{}l@{}}=\\ 1\end{tabular}                                                                   & \cmark                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      \\ \hline
2                                                   & Use limited data to select advertising                                                 & New Looks new language but related to P 2 = “Select basic ads”       & \cmark                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      \\ \hline
3                                                   & Create profiles for personalised advertising                                           & \begin{tabular}[c]{@{}l@{}}=\\ 3\end{tabular}                                                                   & \cmark                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      \\ \hline
4                                                   & Use profiles to select personalised advertising                                        & \begin{tabular}[c]{@{}l@{}}=\\ 4\end{tabular}                                                                   & \cmark                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      \\ \hline
\begin{tabular}[c]{@{}l@{}}5\\ (and 6)\end{tabular} & Create profiles to personalise content                                                 & \begin{tabular}[c]{@{}l@{}}=\\ 5\end{tabular}                                                                   & (\cmark) Not clear: in principle, this P can be legitimized under a legitimate interest, but it would fail the LI test. However, according to Recital 47 of the GPDR, when using legitimate interest as a legal basis for processing, the controller (in the balance test) has to consider the reasonable expectations of data subjects based on their relationship with the controller. This expectation must exist at the time and in the context of the collection of her personal data. Meanwhile, the collection of data from unknown sources, by third-parties that users have never heard of and do not have a direct relationship with – to profile them and share these “insights” with other advertisers – is not plausibly within the individuals’ reasonable expectations. Hence, we suppose that processing personal data of users that have no relationship with third-party advertisers, which is the case in the TCF, will, in practice, make that balance weight towards the interest and rights of users. As posited by the Norwegian Consumer Council , “although consumers may know that many “free” digital services are funded by advertising, this does not mean that most people will have a “reasonable expectation” of the amount of sharing and processing going on behind the scenes (...) Companies are virtually unknown to most consumers, so one can hardly consider this a relationship at all.” Thus, the potentially unique purpose (from the specification of the TCF) that would rely on legitimate interest could, in practice, fail the requirements of such a legal basis. \\ \hline
6                                                   & Use profiles to select personalised content                                            & \begin{tabular}[c]{@{}l@{}}=\\ 6\end{tabular}                                                                   & (\cmark) Not clear: in principle, this P can be legitimized under a legitimate interest, but it would fail the LI test (see reasoning above)                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                \\ \hline
7                                                   & Measure advertising performance                                                        & \begin{tabular}[c]{@{}l@{}}=\\ 7\end{tabular}                                                                   & \cmark                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      \\ \hline
8                                                   & Measure content performance                                                            & \begin{tabular}[c]{@{}l@{}}=\\ 8\end{tabular}                                                                   & \cmark                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      \\ \hline
9                                                   & Understand audiences through statistics or combinations of data from different sources & New language but Looks like the former one (P number 9) ‘’Apply market research to generate audience insights’’ & \cmark                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      \\ \hline
10                                                  & Develop and improve services                                                           & \begin{tabular}[c]{@{}l@{}}= \\ 10\end{tabular}                                                                 & It is not specific, and so we cannot derive its legal basis.  X but in principle it could rely on LI though it could fail the LI test                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     \\ \hline
11                                                  & Use limited data to select content                                                     & New                                                                                                             & X                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      \\ \hline
\end{tabular}
% \end{longtable}
% \twocolumn
\end{table*}

==> tables/table1.tex <==
\begin{table}[]

\begin{tabular}{|l|c|c|}
\hline
  \textbf{}      & % & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}l@{}}Total Reachable \\ Websites\end{tabular}}} &
                                                                                                                        % W. RO & W/O RO \\ \hline 
  \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Websites with \\ Revocation \\ Options\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Websites without \\ Revocation \\Options\end{tabular}}} \\ \hline
  \textbf{Consent Banner}   %& 111 (65\%)
                                                                                                                       & 97 (56.7\%)                                                                                               & 14  (8\%)                                                                                                \\ \hline
  \textbf{Consent Notice}  %& 6 (4\%)
                                                                                                                       & 4  (2.3\%)                                                                                               & 3  (2\%)                                                                                                                                                                                                \\ \hline
  \textbf{No Banner or Notice} %& 53 (31\%)
                                                                                                                       & 14 (8.7\%)                                                                                               & 39   (22.8\%)                                                                                                \\ \hline
\end{tabular}
\caption{Number of websites with banners, notices and no initial pop-ups displaying consent modification options. The numbers in brackets are the percentage of websites from the \euw reachable websites.}
\label{tab:banner_rev}
\end{table}

==> tables/table10.tex <==
\begin{table*}[h]
  \begin{adjustbox}{width=\linewidth}
  
  \begin{tabular}{|lllll|}
  \hline
  \multicolumn{1}{|l|}{\textbf{Phase}}   & \multicolumn{1}{l|}{\textbf{Source}} & \multicolumn{1}{l|}{\textbf{Responsible party}}                                                                                                                   & \multicolumn{1}{l|}{\textbf{Website (Rank)}}            & \textbf{Comments}                                                                                                                                                                                                                                      \\ \hline
  \multicolumn{5}{|c|}{Inconsistencies due to delay in updating the consent after user revokes consent}                                                                                                                                                                                                                                                                                                                                                                                                                                                                \\ \hline
  \multicolumn{1}{|l|}{After Acceptance} & \multicolumn{1}{l|}{Request}         & \multicolumn{1}{l|}{Third-party domain}                                                                                                                           & \multicolumn{1}{l|}{cnn.com (91)}                       & Difference of 10 seconds before the updated consent is sent in the request.                                                                                                                                                                            \\ \hline
  \multicolumn{1}{|l|}{After Acceptance} & \multicolumn{1}{l|}{Request}         & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Third-party domain (GTM \\ and Host) and First-party domain\end{tabular}}                                          & \multicolumn{1}{l|}{http://independent.co.uk (210)}     & Cookie updated but URL parameter wasn't updated till 1.07s.                                                                                                                                                                                            \\ \hline
  \multicolumn{1}{|l|}{After Acceptance} & \multicolumn{1}{l|}{Request}         & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Third-party script loaded by\\  first-party on initial landing\end{tabular}}                                       & \multicolumn{1}{l|}{marca.com (544)}                    & \begin{tabular}[c]{@{}l@{}}"iabconsent" variable not updated but "gdpr\_consent" variable updated in\\  the URL query parameters. It was later updated in 1.44 seconds.\end{tabular}                                                                   \\ \hline
  \multicolumn{1}{|l|}{After Acceptance} & \multicolumn{1}{l|}{Request}         & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Third-party script loaded by\\ third-party script loaded by\\ first-party privacy management script.\end{tabular}} & \multicolumn{1}{l|}{lavozdegalicia.es (3592)}           & \begin{tabular}[c]{@{}l@{}}"iabconsent" variable not updated but "gdpr\_consent" variable updated in \\ the URL query parameters. It was later updated in 0.99 seconds.\end{tabular}                                                                   \\ \hline
  \multicolumn{1}{|l|}{After Acceptance} & \multicolumn{1}{l|}{Request}         & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Third-party script loaded by\\ third-party script loaded by\\ first-party privacy management script.\end{tabular}} & \multicolumn{1}{l|}{klix.ba (4566)}                     & \begin{tabular}[c]{@{}l@{}}"iabconsent" variable not updated but "gdpr\_consent" variable updated in \\ the URL query parameters. It was later updated in 2 seconds.\end{tabular}                                                                      \\ \hline
  \multicolumn{1}{|l|}{After Revocation} & \multicolumn{1}{l|}{Request}         & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Third-party script loaded by\\ a third-party script\end{tabular}}                                                  & \multicolumn{1}{l|}{idnes.cz (581)}                     & \begin{tabular}[c]{@{}l@{}}POST data with different variables with different consents and took 16 \\ seconds for all variables to be updated.\end{tabular}                                                                                             \\ \hline
  \multicolumn{5}{|c|}{Inconsistencies due to using an altogether different TCString}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                  \\ \hline
  \multicolumn{1}{|l|}{After Acceptance} & \multicolumn{1}{l|}{Response}        & \multicolumn{1}{l|}{Third-party domain (CMP)}                                                                                                                     & \multicolumn{1}{l|}{forbes.com (87)}                    & Vendor list and vendor purposes increased.                                                                                                                                                                                                             \\ \hline
  \multicolumn{1}{|l|}{After Revocation} & \multicolumn{1}{l|}{Response}        & \multicolumn{1}{l|}{Third-party domain (CMP)}                                                                                                                     & \multicolumn{1}{l|}{forbes.com (87)}                    & Vendor list and vendor purposes increased.                                                                                                                                                                                                             \\ \hline
  \multicolumn{1}{|l|}{After Acceptance} & \multicolumn{1}{l|}{Response}        & \multicolumn{1}{l|}{Third-party domain (CMP)}                                                                                                                     & \multicolumn{1}{l|}{time.com (208)}                     & \begin{tabular}[c]{@{}l@{}}Vendor list and and vendor purposes increased. Different number of active\\ purposes. 13 different TCStrings.\end{tabular}                                                                                                  \\ \hline
  \multicolumn{1}{|l|}{After Revocation} & \multicolumn{1}{l|}{Response}        & \multicolumn{1}{l|}{Third-party domain (CMP)}                                                                                                                     & \multicolumn{1}{l|}{time.com (208)}                     & \begin{tabular}[c]{@{}l@{}}Vendor list and and vendor purposes increased. Different number of active\\ purposes. 13 different TCStrings.\end{tabular}                                                                                                  \\ \hline
  \multicolumn{1}{|l|}{After Revocation} & \multicolumn{1}{l|}{Request}         & \multicolumn{1}{l|}{First-party domain}                                                                                                                           & \multicolumn{1}{l|}{n-tv.de (550)}                      & \begin{tabular}[c]{@{}l@{}}Consent string received from hardcoded code from first party then sent to \\ third party. Purpose legitimate interests (5) and vendor legitimate \\ interests(3) added.\end{tabular}                                        \\ \hline
  \multicolumn{1}{|l|}{After Acceptance} & \multicolumn{1}{l|}{Response}        & \multicolumn{1}{l|}{Third-party domain (CMP)}                                                                                                                     & \multicolumn{1}{l|}{cadenaser.com (3059)}               & \begin{tabular}[c]{@{}l@{}}Variable storing a different TCString in the response sent by TP called by \\ a TP script when an updated TCString was sent in the request.\end{tabular}                                                                    \\ \hline
  \multicolumn{5}{|c|}{Inconsistencies in the scripts not being updated about user revoking consent}                                                                                                                                                                                                                                                                                                                                                                                                                                                                   \\ \hline
  \multicolumn{1}{|l|}{After Revocation} & \multicolumn{1}{l|}{Request}         & \multicolumn{1}{l|}{First-party}                                                                                                                                  & \multicolumn{1}{l|}{deadline.com (2061)}                & Updated consent not shared in the network.                                                                                                                                                                                                             \\ \hline
  \multicolumn{1}{|l|}{After Acceptance} & \multicolumn{1}{l|}{Request}         & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Third-party script loaded by \\ first-party on initial landing\end{tabular}}                                       & \multicolumn{1}{l|}{kotaku.com (3047)}                  & \begin{tabular}[c]{@{}l@{}}The correct consent was being sent in the URL and cookie, but this script\\ sent the old consent even after 1.5 seconds. No other request was sent later\\ by this script to check if the consent was updated.\end{tabular} \\ \hline
  \multicolumn{1}{|l|}{After Revocation} & \multicolumn{1}{l|}{Request}         & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Third-party script loaded by\\ first party\end{tabular}}                                                           & \multicolumn{1}{l|}{kotaku.com (3047)}                  & \begin{tabular}[c]{@{}l@{}}Third-party script was loaded after the consent was updated, but it still \\ used the wrong consent after 16 seconds.\end{tabular}                                                                                          \\ \hline
  \multicolumn{1}{|l|}{After Revocation} & \multicolumn{1}{l|}{Request}         & \multicolumn{1}{l|}{Third-party script}                                                                                                                           & \multicolumn{1}{l|}{manchestereveningnews.co.uk (3569)} & \begin{tabular}[c]{@{}l@{}}Updated consent was sent in the network. But \\ signal-beacon.s-onetag.com/beacon.min.js sends the old consent.\end{tabular}                                                                                                \\ \hline
  \multicolumn{1}{|l|}{After Revocation} & \multicolumn{1}{l|}{Request}         & \multicolumn{1}{l|}{Third-party script}                                                                                                                           & \multicolumn{1}{l|}{walesonline.co.uk (4093)}           & \begin{tabular}[c]{@{}l@{}}Updated consent was sent in the network. But\\ signal-beacon.s-onetag.com/beacon.min.js sends the old consent.\end{tabular}                                                                                                 \\ \hline
  \end{tabular}
      
  \end{adjustbox}
  \caption{Inconsistencies in the network}
  \label{app-tab:anomaly2}
  \end{table*}

% \NBcom{Please fix the table~\ref{tab:anomaly2}, don't use {adjustbox} and don't put tabular inside the cells. The font inside the tables must be the same as the main paper. This type of fixes can be considered as attempts to gain space and we can easily get a desk reject because of bad formatting of our paper. I fixed many of the tables already, but please fix others if you see this again.}


% \caption{Inconsistencies in the responses received in the network}
% \label{tab:anomaly2}

% \end{table*}

==> tables/table11.tex <==
% \NBcom{remove first column of Table 11}

\begin{table}[]
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{|p{2cm}|p{1cm}|p{2cm}|p{2cm}|}
\hline
\textbf{Third- parties informed}         & \textbf{No.of Websites} & \textbf{No.of websites sending non-empty string after revocation (third-parties receiving the string)} & \textbf{No.of websites sending empty string after revocation (third-parties receiving the string)} \\ \hline
Atleast one third-party was informed     & 61                      & 6 (160 third-parties)                                                                                  & 55 (79 third-parties)                                                                              \\ \hline
Atleast one third-party was not informed & 101                     & 13 (1302 third-parties)                                                                                & 88 (148 third-parties)                                                                             \\ \hline
\end{tabular}
\end{adjustbox}
\caption{Third-parties}
\label{tab:third-parties}
\end{table}


% \begin{tabular}{|p{2.5cm}|p{2.1cm}|p{2.4cm}|}
% \hline
% \textbf{Browser storage types and API} & 
% \textbf{Number of websites} & 
% \textbf{Examples of allowed purposes}
% \\ \hline
% cookies                                           
% & 8  (out of 100)      & INSERT
% \\ \hline
% localStorage         
% & 4  (out of 32)  &  INSERT
% \\ \hline
% \tcfapi                                        
% & 16 (out of 136)  & INSERT
% \\ \hline
% \end{tabular}

==> tables/table9.tex <==



\begin{table}[]
\begin{tabular}{|lllll|}
\hline
\multicolumn{1}{|l|}{\textbf{Phase}}   & \multicolumn{1}{l|}{\textbf{Source}} & \multicolumn{1}{l|}{\textbf{Responsible party}}                                                                                                                   & \multicolumn{1}{l|}{\textbf{Website (Rank)}}            & \textbf{Comments}                                                                                                                                                                                                                                      \\ \hline
\multicolumn{5}{|c|}{Inconsistencies due to delay in updating the consent after user revokes consent}                                                                                                                                                                                                                                                                                                                                                                                                                                                                \\ \hline
\multicolumn{1}{|l|}{After Acceptance} & \multicolumn{1}{l|}{Request}         & \multicolumn{1}{l|}{Third-party domain}                                                                                                                           & \multicolumn{1}{l|}{cnn.com (91)}                       & Difference of 10 seconds before the updated consent is sent in the request.                                                                                                                                                                            \\ \hline
\multicolumn{1}{|l|}{After Acceptance} & \multicolumn{1}{l|}{Request}         & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Third-party domain (GTM \\ and Host) and First-party domain\end{tabular}}                                          & \multicolumn{1}{l|}{http://independent.co.uk (210)}     & Cookie updated but URL parameter wasn't updated till 1.07s.                                                                                                                                                                                            \\ \hline
\multicolumn{1}{|l|}{After Acceptance} & \multicolumn{1}{l|}{Request}         & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Third-party script loaded by\\  first-party on initial landing\end{tabular}}                                       & \multicolumn{1}{l|}{marca.com (544)}                    & \begin{tabular}[c]{@{}l@{}}"iabconsent" variable not updated but "gdpr\_consent" variable updated in\\  the URL query parameters. It was later updated in 1.44 seconds.\end{tabular}                                                                   \\ \hline
\multicolumn{1}{|l|}{After Acceptance} & \multicolumn{1}{l|}{Request}         & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Third-party script loaded by \\ first-party on initial landing\end{tabular}}                                       & \multicolumn{1}{l|}{kotaku.com (3047)}                  & \begin{tabular}[c]{@{}l@{}}The correct consent was being sent in the URL and cookie, but this script\\ sent the old consent even after 1.5 seconds. No other request was sent later\\ by this script to check if the consent was updated.\end{tabular} \\ \hline
\multicolumn{1}{|l|}{After Acceptance} & \multicolumn{1}{l|}{Request}         & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Third-party script loaded by\\ third-party script loaded by\\ first-party privacy management script.\end{tabular}} & \multicolumn{1}{l|}{lavozdegalicia.es (3592)}           & \begin{tabular}[c]{@{}l@{}}"iabconsent" variable not updated but "gdpr\_consent" variable updated in \\ the URL query parameters. It was later updated in 0.99 seconds.\end{tabular}                                                                   \\ \hline
\multicolumn{1}{|l|}{After Acceptance} & \multicolumn{1}{l|}{Request}         & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Third-party script loaded by\\ third-party script loaded by\\ first-party privacy management script.\end{tabular}} & \multicolumn{1}{l|}{klix.ba (4566)}                     & \begin{tabular}[c]{@{}l@{}}"iabconsent" variable not updated but "gdpr\_consent" variable updated in \\ the URL query parameters. It was later updated in 2 seconds.\end{tabular}                                                                      \\ \hline
\multicolumn{1}{|l|}{After Revocation} & \multicolumn{1}{l|}{Request}         & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Third-party script loaded by\\ a third-party script\end{tabular}}                                                  & \multicolumn{1}{l|}{idnes.cz (581)}                     & \begin{tabular}[c]{@{}l@{}}POST data with different variables with different consents and took 16 \\ seconds for all variables to be updated.\end{tabular}                                                                                             \\ \hline
\multicolumn{1}{|l|}{After Revocation} & \multicolumn{1}{l|}{Request}         & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Third-party script loaded by\\ first party\end{tabular}}                                                           & \multicolumn{1}{l|}{kotaku.com (3039)}                  & \begin{tabular}[c]{@{}l@{}}Third-party script was loaded after the consent was updated, but it still \\ used the wrong consent after 16 seconds.\end{tabular}                                                                                          \\ \hline
\multicolumn{5}{|c|}{Inconsistencies due to using an altogether different TCString}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                  \\ \hline
\multicolumn{1}{|l|}{After Acceptance} & \multicolumn{1}{l|}{Response}        & \multicolumn{1}{l|}{Third-party domain (CMP)}                                                                                                                     & \multicolumn{1}{l|}{forbes.com (87)}                    & Vendor list and vendor purposes increased.                                                                                                                                                                                                             \\ \hline
\multicolumn{1}{|l|}{After Revocation} & \multicolumn{1}{l|}{Response}        & \multicolumn{1}{l|}{Third-party domain (CMP)}                                                                                                                     & \multicolumn{1}{l|}{forbes.com (87)}                    & Vendor list and vendor purposes increased.                                                                                                                                                                                                             \\ \hline
\multicolumn{1}{|l|}{After Acceptance} & \multicolumn{1}{l|}{Response}        & \multicolumn{1}{l|}{Third-party domain (CMP)}                                                                                                                     & \multicolumn{1}{l|}{time.com (208)}                     & \begin{tabular}[c]{@{}l@{}}Vendor list and and vendor purposes increased. Different number of active\\ purposes. 13 different TCStrings.\end{tabular}                                                                                                  \\ \hline
\multicolumn{1}{|l|}{After Revocation} & \multicolumn{1}{l|}{Response}        & \multicolumn{1}{l|}{Third-party domain (CMP)}                                                                                                                     & \multicolumn{1}{l|}{time.com (208)}                     & \begin{tabular}[c]{@{}l@{}}Vendor list and and vendor purposes increased. Different number of active\\ purposes. 13 different TCStrings.\end{tabular}                                                                                                  \\ \hline
\multicolumn{1}{|l|}{After Revocation} & \multicolumn{1}{l|}{Request}         & \multicolumn{1}{l|}{First-party domain}                                                                                                                           & \multicolumn{1}{l|}{n-tv.de (550)}                      & \begin{tabular}[c]{@{}l@{}}Consent string received from hardcoded code from first party then sent to \\ third party. Purpose legitimate interests (5) and vendor legitimate \\ interests(3) added.\end{tabular}                                        \\ \hline
\multicolumn{1}{|l|}{After Acceptance} & \multicolumn{1}{l|}{Response}        & \multicolumn{1}{l|}{Third-party domain (CMP)}                                                                                                                     & \multicolumn{1}{l|}{cadenaser.com (3059)}               & \begin{tabular}[c]{@{}l@{}}Variable storing a different TCString in the response sent by TP called by \\ a TP script when an updated TCString was sent in the request.\end{tabular}                                                                    \\ \hline
\multicolumn{5}{|c|}{Inconsistencies in the scripts not being updated about user revoking consent}                                                                                                                                                                                                                                                                                                                                                                                                                                                                   \\ \hline
\multicolumn{1}{|l|}{After Revocation} & \multicolumn{1}{l|}{Request}         & \multicolumn{1}{l|}{First-party}                                                                                                                                  & \multicolumn{1}{l|}{deadline.com (2061)}                & Updated consent not shared in the network.                                                                                                                                                                                                             \\ \hline
\multicolumn{1}{|l|}{After Revocation} & \multicolumn{1}{l|}{Request}         & \multicolumn{1}{l|}{Third-party script}                                                                                                                           & \multicolumn{1}{l|}{manchestereveningnews.co.uk (3569)} & \begin{tabular}[c]{@{}l@{}}Updated consent was sent in the network. But \\ signal-beacon.s-onetag.com/beacon.min.js sends the old consent.\end{tabular}                                                                                                \\ \hline
\multicolumn{1}{|l|}{After Revocation} & \multicolumn{1}{l|}{Request}         & \multicolumn{1}{l|}{Third-party script}                                                                                                                           & \multicolumn{1}{l|}{walesonline.co.uk (4093)}           & \begin{tabular}[c]{@{}l@{}}Updated consent was sent in the network. But\\ signal-beacon.s-onetag.com/beacon.min.js sends the old consent.\end{tabular}                                                                                                 \\ \hline
\end{tabular}
\end{table}

% \caption{Inconsistencies in the requests sent in the network}
% \label{tab:anomaly1}
% \end{table*}


% \end{table*}

==> tables/table_cat_wise.tex <==
\begin{table}[]
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{|l|r|r|r|r|r|lr|lr|lr|lr|}
\hline
                               & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Total no.of \\ websites(171)\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Revocation \\ possible(114)\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Banner with \\ revocation (97)\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Notice with \\ revocation (3)\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}No banner with\\  revocation (14)\end{tabular}}} & \multicolumn{2}{l|}{\textbf{Initial}}                                 & \multicolumn{2}{l|}{\textbf{Accept}}                                  & \multicolumn{2}{l|}{\textbf{Revoke}}                                  & \multicolumn{2}{l|}{\textbf{Reject}}                                  \\ \hline
\textbf{Web Categories}        & \multicolumn{1}{l|}{}                                                                              & \multicolumn{1}{l|}{}                                                                             & \multicolumn{1}{l|}{}                                                                                & \multicolumn{1}{l|}{}                                                                               & \multicolumn{1}{l|}{}                                                                                   & \multicolumn{1}{l|}{\textbf{Mean}} & \multicolumn{1}{l|}{\textbf{SD}} & \multicolumn{1}{l|}{\textbf{Mean}} & \multicolumn{1}{l|}{\textbf{SD}} & \multicolumn{1}{l|}{\textbf{Mean}} & \multicolumn{1}{l|}{\textbf{SD}} & \multicolumn{1}{l|}{\textbf{Mean}} & \multicolumn{1}{l|}{\textbf{SD}} \\ \hline
\textbf{Comp \& Int}           & 60                                                                                                 & 41                                                                                                & 35                                                                                                   & 1                                                                                                   & 5                                                                                                       & \multicolumn{1}{l|}{(46)8.82}      & 8.453318869                      & \multicolumn{1}{l|}{(44) 27.06}    & 26.72704326                      & \multicolumn{1}{l|}{(41) 19.6}     & 27.9687                          & \multicolumn{1}{l|}{(46)11.02}     & 9.982858118                      \\ \hline
\textbf{Business \& comm}      & 13                                                                                                 & 9                                                                                                 & 8                                                                                                    & 0                                                                                                   & 1                                                                                                       & \multicolumn{1}{l|}{(12) 12.25}    & 8.628225226                      & \multicolumn{1}{l|}{(11)21.54}     & 19.452177                        & \multicolumn{1}{l|}{(9)18.44}      & 20.2906485                       & \multicolumn{1}{l|}{(12)16.4}      & 10.35788175                      \\ \hline
\textbf{Edu/Research}          & 12                                                                                                 & 3                                                                                                 & 3                                                                                                    & 0                                                                                                   & 0                                                                                                       & \multicolumn{1}{l|}{(6)7.5}        & 11.171276                        & \multicolumn{1}{l|}{(6)21.16}      & 18.31596937                      & \multicolumn{1}{l|}{(3) 22}        & 15.67                            & \multicolumn{1}{l|}{(6)8.6}        & 13.67212198                      \\ \hline
\textbf{Entertainment}         & 14                                                                                                 & 13                                                                                                & 11                                                                                                   & 0                                                                                                   & 2                                                                                                       & \multicolumn{1}{l|}{(13)7.53}      & 8.513066187                      & \multicolumn{1}{l|}{(13) 12.15}    & 19.27269952                      & \multicolumn{1}{l|}{(13)12.25}     & 20.07937783                      & \multicolumn{1}{l|}{(13)9}         & 10.20703122                      \\ \hline
\textbf{File storage /sharing} & \textbf{6}                                                                                         & 3                                                                                                 & 2                                                                                                    & 0                                                                                                   & 1                                                                                                       & \multicolumn{1}{l|}{(3) 7.666}     & 8.178779915                      & \multicolumn{1}{l|}{(3) 10.33}     & 19.83751111                      & \multicolumn{1}{l|}{(3) 9.33}      & 20.89537785                      & \multicolumn{1}{l|}{(3)8}          & 11.31999618                      \\ \hline
\textbf{Gov/heal/legal}        & 8                                                                                                  & 3                                                                                                 & 2                                                                                                    & 0                                                                                                   & 1                                                                                                       & \multicolumn{1}{l|}{(3)7}          & 8.906711413                      & \multicolumn{1}{l|}{(3) 13}        & 29.25415418                      & \multicolumn{1}{l|}{(3)12.33}      & 18.12703413                      & \multicolumn{1}{l|}{(3)8.33}       & 12.34645024                      \\ \hline
\textbf{News/Forums}           & 23                                                                                                 & 16                                                                                                & 14                                                                                                   & 1                                                                                                   & 1                                                                                                       & \multicolumn{1}{l|}{(20) 14.3}     & 8.979172117                      & \multicolumn{1}{l|}{(18)39.33}     & 27.90986961                      & \multicolumn{1}{l|}{(16) 32.25}    & 31.40925064                      & \multicolumn{1}{l|}{(20)16.44}     & 10.85651379                      \\ \hline
\textbf{Social media/net}      & 13                                                                                                 & 10                                                                                                & 8                                                                                                    & 0                                                                                                   & 2                                                                                                       & \multicolumn{1}{l|}{(10)5.2}       & 8.644742101                      & \multicolumn{1}{l|}{(10) 15.7}     & 19.55148379                      & \multicolumn{1}{l|}{(10) 11.1}     & 20.37011012                      & \multicolumn{1}{l|}{(10)6.5}       & 10.23369958                      \\ \hline
Web                            & 22                                                                                                 & 16                                                                                                & 14                                                                                                   & 1                                                                                                   & 1                                                                                                       & \multicolumn{1}{l|}{(19)6.63}      & 8.478054639                      & \multicolumn{1}{l|}{(19) 20.89}    & 26.80297587                      & \multicolumn{1}{l|}{(16)18.81}     & 28.09979648                      & \multicolumn{1}{l|}{(19)8.77}      & 10.11469466                      \\ \hline
\end{tabular}
\label{tab:cat_wise}
\end{adjustbox}
\end{table}

